Information Farming: From Berry Picking to Berry Growing

The classic paradigms of Berry Picking and Information Foraging Theory have framed users as gatherers, opportunistically searching across distributed sources to satisfy evolving information needs. However, the rise of GenAI is driving a fundamental transformation in how people produce, structure, and reuse information - one that these paradigms no longer fully capture. This transformation is analogous to the Neolithic Revolution, when societies shifted from hunting and gathering to cultivation. Generative technologies empower users to "farm" information by planting seeds in the form of prompts, cultivating workflows over time, and harvesting richly structured, relevant yields within their own plots, rather than foraging across others people's patches. In this perspectives paper, we introduce the notion of Information Farming as a conceptual framework and argue that it represents a natural evolution in how people engage with information. Drawing on historical analogy and empirical evidence, we examine the benefits and opportunities of information farming, its implications for design and evaluation, and the accompanying risks posed by this transition. We hypothesize that as GenAI technologies proliferate, cultivating information will increasingly supplant transient, patch-based foraging as a dominant mode of engagement, marking a broader shift in human-information interaction and its study.

==> tables/timeline.tex <==
\renewcommand{\arraystretch}{1.3} % extra row spacing
\setlength{\tabcolsep}{8pt} % column spacing
\begin{table*}[htbp]
\centering
\renewcommand{\arraystretch}{1.2} % row spacing
\setlength{\tabcolsep}{6pt} % column spacing
\begin{tabular}{|c|c|c|}
\hline
\textbf{Year} & \textbf{Model Name} & \textbf{Description} \\
\hline
1980 & Anomalous State of Knowledge (ASK) & Belkin’s model describing an information need as an anomaly or gap in the seeker’s knowledge. \\
\hline
1981 & General Model of Information Behaviour & Wilson’s framework showing how context and barriers lead to information needs and seeking behavior. \\
\hline
1983 & Sense-Making (Gap-Bridging) & Dervin’s metaphor of users bridging a gap in understanding to move from confusion to sense. \\
\hline
1980s & Pearl Growing & Starting with one 'seed' document and iteratively expanding outward to grow a collection. \\
\hline
1989 & Berry-Picking Model & Bates’s analogy of gathering information in bits, like picking berries one by one along a meandering path. \\
\hline
1989 & Ellis’s Behavioral Model & Ellis identifies activities like starting, chaining, browsing, etc., as flexible patterns in information seeking. \\
\hline
1991 & Kuhlthau’s ISP (Uncertainty Principle) & Six-stage model noting users’ uncertainty and anxiety in early stages, giving way to clarity later. \\
\hline
1993 & Orienteering (vs. Teleporting) & O’Day \& Jeffries’s notion of users navigating stepwise through information rather than jumping directly to answers. \\
\hline
1995 & Domain Analysis \& ``Information Horizons'' & Hjørland’s approach focusing on subject domains; users navigate within a domain-specific information space. \\
\hline
1995 & Everyday Life Information Seeking (ELIS) & Savolainen’s model emphasizing how one’s way of life and daily context shape information seeking. \\
\hline
1997 & Information Encountering & Erdelez’s concept of serendipitous discovery: ``bumping into'' useful information while not actively seeking it. \\
\hline
1999 & Information Foraging Theory & Pirolli \& Card’s analogy of users as foraging animals, following information ``scent'' to find useful information. \\
\hline
1999 & Information Grounds & Pettigrew’s metaphor of places where people gather for other purposes but end up sharing information informally. \\
\hline
2000s & Wayfinding \& Info Space & Users as travellers navigating information spaces using landmarks, paths, and maps. \\
\hline
2007 & Knowledge Gardening & Gardening metaphor: planting ideas, cultivating knowledge, weeding out old info, and harvesting insights. \\
\hline
2008 & Fishing for Information & The metaphor of fishing: casting broad queries and hoping to catch useful information. \\
\hline
2009 & Tetris Model & Max Wilson’s analogy likening searching to playing Tetris: fitting pieces of information together to resolve different aspects. \\
\hline
2011 & Search as Economic Activity & Azzopardi’s economic model of search, treating users as rational actors balancing costs and benefits. \\
\hline
2015 & Card-Playing Model & Chengxiang Zhai’s model of search as a card game, where the system and user take turns in an interactive retrieval session. \\
\hline
2010s & Search as Conversation & Search as a multi-turn dialogue between the user and system to clarify needs and retrieve information iteratively. \\
\hline
\end{tabular}
\caption{Timeline of Information Behaviour Models}
\end{table*}
